Ethics, Rules of Engagement, and AI: Neural Narrative Mapping Using Large Transformer Language Models

The problem of determining if a military unit has correctly understood an order and is properly executing on it is one that has bedeviled military planners throughout history. The advent of advanced language models such as OpenAI's GPT-series offers new possibilities for addressing this problem. This paper presents a mechanism to harness the narrative output of large language models and produce diagrams or "maps" of the relationships that are latent in the weights of such models as the GPT-3. The resulting "Neural Narrative Maps" (NNMs), are intended to provide insight into the organization of information, opinion, and belief in the model, which in turn provide means to understand intent and response in the context of physical distance. This paper discusses the problem of mapping information spaces in general, and then presents a concrete implementation of this concept in the context of OpenAI's GPT-3 language model for determining if a subordinate is following a commander's intent in a high-risk situation. The subordinate's locations within the NNM allow a novel capability to evaluate the intent of the subordinate with respect to the commander. We show that is is possible not only to determine if they are nearby in narrative space, but also how they are oriented, and what "trajectory" they are on. Our results show that our method is able to produce high-quality maps, and demonstrate new ways of evaluating intent more generally.

==> text/author_instructions.tex <==
\section{Author Instructions}

Dear Phil,
 
Thank you again for accepting our invitation to submit a paper to the IEEE Data Engineering Bulletin special issue on Responsive AI and HCI.  We wanted to check in with details on how to submit to the special issue.  
 

Please submit your paper for review in PDF format via the EasyChair service at the link below.  The formatting requirements are given below under “Author instructions.”  Note that the publishers require that the papers are created using the LaTeX document preparation system using the attached style file.  We realize that since this is an interdisciplinary issue this may not be ideal for some authors.  We will not enforce these requirements in your original submission due Dec. 10 (e.g., your original submission can be created in MS Word), but we will need to have a LaTeX version that complies with the requirements for the camera-ready copy, due December 22.  If this presents a problem for your team, please let us know and we are here to help.

 

Our apologies about the broken link to deauthor.sty in the Data Engineering Bulletin author instructions page(\url{http://tab.computer.org/tcde/bull_author.html}).  I have attached the LaTeX style file, called deauthor.sty, and an example tex file which can be used as a template.  Note the following points which are stated in the author instructions:

 

- Your paper must be contained in a single tex file.

 

- The paper must be in a folder named after the author(s)

 

- Figures must be included in a subfolder called “figs”

 

- Bibliography entries need to be included in the tex file (i.e., you can’t use BibTeX, unfortunately). Note that although you can't use Bibtex, there is a simple workaround: you can simply compile with bibtex on your end then paste the .bbl file that bibtex creates into your tex file.  We only need the latex source for the final camera-ready version.

 

- Please only include packages that you actually use.  This is to prevent unnecessary conflicts when we combine all accepted papers’ files into a single issue.

 

- You will need to compile using the latex -> DVI -> PDF command pipeline rather than using pdflatex, otherwise compilation will fail once you include any figures.  This command pipeline can usually be chosen in the settings for your LaTeX editor.  If you cannot compile the template file attached, please verify that you are doing this.  As a temporary workaround for your initial submission, you could comment out the first line of the template file and replace it with “documentclass[11pt]{article}”, which will make it possible to compile with pdflatex.  This workaround also seems to be necessary if you edit your paper using Overleaf.

 

Please see below for the deadlines and links.  If you have any questions, feel free to let us know.

 

Shimei Pan and James Foulds.

 

===============================================================

Updated submission deadlines:

Submission deadline Dec. 10th (PDF copy, submit using EasyChair)

Review feedback: Dec. 15th

Camera Ready deadline: Dec 22 (LaTeX source code which complies with the author instructions, submit using email)

 

Author instructions: \url{http://tab.computer.org/tcde/bull_author.html}

 

Easy Chair Submission link:  \url{https://easychair.org/conferences/?conf=debdec2021}


Page limit: 12 pages in a single-column IEEE format (Soft Constraint).

==> text/biographies.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}{Philip Feldman}
Biography text here.
\end{IEEEbiography}

% if you will not have a photo at all: 
\begin{IEEEbiographynophoto}{Aaron Dant}
Biography text here.
\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiographynophoto}{David Rosenbluth}
Biography text here.
\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}

==> text/enhanced_sim.tex <==
\section{Enhanced Simulation}
Enhanced simulation means that ML can explore \textit{tactical} options

Deliver the right amount of energy in the right place for the lowest cost(?)

==> text/notes.tex <==
\section{notes}

Topics as well as their containing nodes need to be able to point to each other. This allows for later evaluation of the manual clustering, as well as opening up the possibilities to explore different clustering, as well as in-node \textit{submaps}. This means that the topic of \enquote{kill} can be associated with the belief about the appropriate rules of engagement, and then further divided into subtopics like \enquote{in combat} , \enquote{manifesting hostility}, etc.

\begin{comment}
\TODO{Tell the story better}
To return to our example from \textit{Apocalypse Now}, we may now have an approach that would have discovered far earlier Col. Kurtz' drift into madness. More importantly, at scale this approach might have been able to detect poor decisions in US policy in Vietnam that led to the loss of that country to the North Vietnamese, and more recently the loss of Afghanistan to the Taliban.


		ON TAPE
"11th transmission, December 30th, 0500 hours, sector KZK."

		KURTZ (on tape)
"but we must kill them. We must incinerate them. Pig after pig, cow after cow, village after village, army after army. And they call me an assassin. What do you call it when the assassins accuse the assassin ? They lie.. they lie and we have to be merciful for those who lie. Those nabobs. I hate them. How I hate them..."

		CORMAN
"Walt Kurtz was one of the most outstanding officers this country has ever produced. He was brilliant. He was outstanding in every way and he was a good man too. Humanitarian man. A man of wit, of humor. He joined the Special forces. And after that his ideas, methods... became... unsound... unsound."

		LUCAS
"Now he's crossed to Cambodia with his Montagnard army of his, who worship the man, like a god, and follow every order however ridiculous."

		CORMAN
"Well, I have some other shocking news to tell you. Colonel Kurtz was about to be arrested for murder."

		WILLARD
"I don't follow sir. Murdered who?"

		LUCAS
"Kurtz had ordered executions of some Vietnamese intelligence agents. Men he believed were double agents. So he took matters into his own hands."

		CORMAN
"Well, you see Willard... In this war, things get confused out there. Power, ideals, the old morality, and practical military necessity. But out there with these natives it must be a temptation to be god. Because there's a conflict in every human heart. Between the rational and the irrational, between  good and  evil. The  good does not always triumph. Sometimes the dark side overcomes what Lincoln called the better angels of our nature. Every man has got a breaking point. You and I have. Walt Kurtz has reached his.  And very obviously, he has gone insane."

		WILLARD
"Yes sir, very much so sir. Obviously insane."

		LUCAS
"Your mission is to proceed up to Nung river in a Navy patrol boat. Pick up colonel Kurtz' path at Nu Mung Ba, follow it, learn what you can along the way. When you find colonel infiltrate his team by whatever means available and terminate the colonel's command."

		WILLARD
"Terminate? The colonel?"

		CORMAN
"He's out there operating without any decent restraint. Totally beyond the pale of any acceptable human conduct. And he is still in the field commanding his troops."

		CIVILIAN
"Terminate with extreme prejudice."

		LUCAS
"You understand captain, that this operation does not exist, nor will it ever exist."

\end{comment}

==> text/response.tex <==
\section*{response}

Dear Philip,

we are delighted to inform you that the following submission has been accepted to appear at the IEEE Data Engineering Bulletin December 2021 issue:

3: Ethics, Rules of Engagement, and AI: Mapping and Locating Beliefs Using Large Transformer Language Models

The review/feedback is also attached here.

Due to the delay in sending out the review, we have decided to extend the camera-ready deadline by one day to Dec. 23.

Congratulations on your fine work! If you have any questions, please feel free to let us know.

Shimei and Jimmy.

SUBMISSION: 3
TITLE: Ethics, Rules of Engagement, and AI: Mapping and Locating Beliefs Using Large Transformer Language Models


----------------------- REVIEW 1 ---------------------

SUBMISSION: 3
TITLE: Ethics, Rules of Engagement, and AI: Mapping and Locating Beliefs Using Large Transformer Language Models
AUTHORS: Philip Feldman, Aaron Dant and David Rosenbluth

----------- Overall evaluation -----------

SCORE: 2 (accept)

----- TEXT:

Paper summary: The paper addresses the problem of understanding whether a military unit has understood and properly executed an order, hence gaining insight into related ethical issues, by way of a methodology for embedding agents and concepts into a "belief space."  An interactive user interface allows an analyst to code different concepts as they occur in dialogue, after which the "belief space" embeddings are updated, and the trajectory in that space can be visualized.  The embeddings are constructed based on responses generated via queries to a GPT language model, which are used to provide input to a force-directed graph layout algorithm.  Demonstrations of the approach are provided on domains with ground truth available (physical maps and philosophy concepts), as well as a military ethics scenario.  The paper also includes interesting discussions on the implications for lethal autonomous weapons systems, and the relationship between human ethics and AI ethics, ultimatel!
 y arguing that in many cases the goal is to increase ethical behavior in humans, in which case bias in AI is actually desirable since it sheds light on human biases.


Quality - Strengths of the paper:

- Understanding and visualizing military ethics and rules of engagement is a new and important problem introduced by the paper, with implications for human ethics, military applications, and potentially, lethal autonomous weapons systems and their associated ethics.

- The paper introduces an innovative strategy for leveraging the semantic knowledge captured by large transformer language models to facilitate semantic understanding. The preliminary results presented here are encouraging.

- The methodology includes an interactive interface in which the human analyst is very much "in the loop" of the underlying AI system, and is able to direct the system to achieve their desired understanding and insights. The dynamic nature of the interactive visualization system aids human understanding and leads to deeper insights than from viewing the data as static.

- The discussions on lethal autonomous weapons and AI bias are insightful and add a new perspective to the conversation in the ethical AI literature.


Quality - Weaknesses of the paper:

- While much of the paper is well written, including beautifully insightful movie analogies and historical examples, the paper could substantially benefit from additional polishing and editing before publication. Specifically:

    (1) There are minor grammatical errors throughout the paper that should be tidied up.

    (2) The framing of the paper could be made more consistent. E.g., the abstract and introduction state that the goal of the work is to understand military orders and ethics, but the future work and conclusions sections say that the paper has achieved the goal of creating belief maps (e.g., Future Work: "We have found that the approach of creating graphical spaces...", "our example was a military one..."; Conclusions: "In this paper, we have shown that creating belief maps...").

    (3) Some of the arguments connecting the different ideas in the paper could be made clearer and stronger. E.g., in both the abstract and the introduction, it isn't immediately clear why advanced language models are likely to be the solution to the problem of determining whether a military unit has understood an order. In both cases, there is a bit of a disconnect between "we want to understand military orders/ethics" and "we are going to use belief space mapping via GPT."


Clarity: See discussion under weaknesses.


Originality and significance: The paper is highly original in that it introduces a new problem, uses transformer language models in an innovative way, and designs a forward-looking human-AI interactive system. It also provides useful insights regarding human ethics and AI ethics, and the relationship between the two.


Scholarship: The Background section could be strengthened by discussing more prior work on "determining intent," including the larger body of prior work which is outside of the relatively new "subordinate vs superior" situation. For transparency, when the authors refer to their own work, they should mention that it is their own work. (There is no double-blind review process so there is no reason not to mention those connections).


Relevance: The paper is very relevant to this special issue.


Minor comments and suggestions to the authors:

- The introduction takes quite a big detour away from introducing and summarizing the paper to go deep into the behavior of GPT, and it never quite fully explains the full argument of the paper.  This makes it difficult for a casual reader to quickly get the main gist of the work without reading the entire paper.  As a suggestion to rectify this, the authors may consider pausing after the first paragraph on page 2 ("indistinguishable from that of humans [4]" to clearly explain the overall argument of the paper and provide an explicit list of its contributions. Then, shift the paper outline here as well ("In this paper, we will discuss...")  Next, shift the discussion on GPT generating text (from "To generate text, the GPT model..." up until almost the end of the introduction) to a new section between Background and Methods.  A connecting sentence could then be added on how you will leverage those properties in the methods section.

- In a similar vein to the above suggestion, the authors may consider having a figure similar to Figure 8 in the first one or two pages so that the reader can see an example of what your method looks like right from the beginning.

- Define "belief space" when the term is first used.  Is this really the best term for this idea?  Usually, I see terms such as "semantic embedding space." If it is a "belief" space, whose beliefs is it representing?  In an AI context, "belief" often refers to the probabilities in Bayesian models, which may be an additional source of confusion regarding this term.

- Depending on your intended audience, you may also want to define or explain the term "pre-trained."

- You may want to distinguish between different senses and uses of the word "bias" throughout the paper.

- Be consistent in the capitalization of "Transformer" (or not capitalizing it).

- Pg 3, "Transformers ... use no pre-defined objective functions" - this statement is not really correct, since the self-supervised tasks do have an objective function.

**Minor grammatical issues:

- Pg 1 "for determine if"; "useful in predicting adjacent and word tokens"

- Pg 2, "The same prompt again and again to produce"

- Pg 3, "subordinates often misunderstand the intent of their superiors 50% - 60% of the time" (delete "often" or otherwise rephrase); "Transformers up many avenues"

- Pg 4, Need a period before "Using this technique"

- Pg 5, `"ground truth",' (comma should go inside quotation marks due to silly historical US English grammar rules that were designed to prevent typewriters from breaking). Figure 3 is referred to before it is described. What does "size of the node" denote?

- Pg 6, I suggest putting prompts in quotation marks (similarly for the other prompts). I'm not sure if this is universal, but the Chicago style manual says to put footnotes after punctuation (footnote 2, footnote 5).

- Pg 7, "a massive corpora" (corpus)

-Pg 10, missing period after "war crime"

-Pg 11, missing period at end of footnote 6

-Pg 12, missing space before "In short, in most scenarios... ."  Consider italicizing "helping humans behave better" since this is such a key point.

-Pg 13, "flexible way of discovering ways" (same word used twice in a row). "SDPs derive from desire path a term in landscape architecture" (missing comma)

-Pg 15 "who's GPT" (whose)

-tidy up capitalization in the references, e.g. "Ai", "bert"



==> text/venues.tex <==
\appendix

\section{Possible Venues}
\begin{itemize}
    \item IEEE International Conference on Systems, Man and Cybernetics: \textit{provides an international forum for researchers and practitioners to report most recent innovations and developments, summarize state-of-the-art, and exchange ideas and advances in all aspects of systems science and engineering, human machine systems, and cybernetics. Advances in these fields have increasing importance in the creation of intelligent environments involving technologies interacting with humans to provide an enriching experience and thereby improve quality of life. Papers related to the conference theme are solicited, including theories, methodologies, and emerging applications. Contributions to theory and practice, including but not limited to the following technical areas, are invited} (example~\cite{roessingh2017machine}) \url{https://ieeesmc.org/}
    \item IEEE Access: \textit{IEEE Access® is a multidisciplinary, applications-oriented, all-electronic archival journal that continuously presents the results of original research or development across all of IEEE's fields of interest. Supported by article processing charges, its hallmarks are a rapid peer review and publication process with open access to all readers.} (example~\cite{wang2020investigation}) \url{https://ieeexplore.ieee.org/xpl/RecentIssue.jsp?punumber=6287639}
    \item The Journal of Defense Modeling and Simulation: Applications, Methodology, Technology: \textit{a quarterly refereed archival journal devoted to advancing the practice, science, and art of modeling and simulation as it relates to the military and defense. The primary focus of the journal is to document, in a rigorous manner, technical lessons derived from practical experience.} (example~\cite{stevens2021can}) \url{https://journals.sagepub.com/home/dms}
\end{itemize}
